PEREGRiNN: Penalized-Relaxation Greedy Neural Network Verifier

Neural Networks (NNs) have increasingly apparent safety implications commensurate with their proliferation in real-world applications: both unanticipated as well as adversarial misclassifications can result in fatal outcomes. As a consequence, techniques of formal verification have been recognized as crucial to the design and deployment of safe NNs. In this paper, we introduce a new approach to formally verify the most commonly considered safety specifications for ReLU NNs -- i.e. polytopic specifications on the input and output of the network. Like some other approaches, ours uses a relaxed convex program to mitigate the combinatorial complexity of the problem. However, unique in our approach is the way we use a convex solver not only as a linear feasibility checker, but also as a means of penalizing the amount of relaxation allowed in solutions. In particular, we encode each ReLU by means of the usual linear constraints, and combine this with a convex objective function that penalizes the discrepancy between the output of each neuron and its relaxation. This convex function is further structured to force the largest relaxations to appear closest to the input layer; this provides the further benefit that the most problematic neurons are conditioned as early as possible, when conditioning layer by layer. This paradigm can be leveraged to create a verification algorithm that is not only faster in general than competing approaches, but is also able to verify considerably more safety properties; we evaluated PEREGRiNN on a standard MNIST robustness verification suite to substantiate these claims.

==> Table_mnist_comparison.tex <==
\begin{table}
\caption{Performance (execution time, number of proved cases) of the three solvers using three different networks. For each cell, the total execution time for the 100 queries is reported together with the number of successfully proved properties. The last column shows the number of properties proved to be safe by PeregeriNN.}
\label{table:Adv_robust}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cc|ccc|c|}
\hline
$\epsilon$ & Architecture&
\begin{tabular}{c}
  Marabou \\
  Time(s) / proved cases
\end{tabular} & 
\begin{tabular}{c}
  Neurify \\
  Time(s) / proved cases
\end{tabular} & \begin{tabular}{c}
  PeregeriNN \\
  Time(s) / proved cases
\end{tabular}
& Safe\\ \hline
1 &
\begin{tabular}{c}
  MNIST\_FC1 \\
  MNIST\_FC2 \\
  MNIST\_FC3
\end{tabular}&
  \begin{tabular}[c]{@{}c@{}}308.8 / \textbf{100} \\ 682.2 / \textbf{100} \\ 38778.5 / 95\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{7.1} / \textbf{100}\\ \textbf{6.37} /\textbf{100}\\ 384 / \textbf{100}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}10 / \textbf{100}\\ 7.806 / \textbf{100}\\ \textbf{91.6} / \textbf{100}\end{tabular}
  &\begin{tabular}[c]{@{}c@{}}97\\99\\100 \end{tabular} \\\hline
5 &
\begin{tabular}{c}
  MNIST\_FC1 \\
  MNIST\_FC2 \\
  MNIST\_FC3
\end{tabular}&
  \begin{tabular}[c]{@{}c@{}}2198.6 / \textbf{100}\\ 41812.13 / 81\\ 1200000 / 0\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}4058.6 / 99\\ 45482.1 / 68\\ 105088.2 / 13\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{595.726} / \textbf{100} \\ \textbf{5921} / \textbf{99} \\ \textbf{39477} / \textbf{71}\end{tabular} &\begin{tabular}[c]{@{}c@{}}77\\86\\69 \end{tabular} \\\hline
10 &
\begin{tabular}{c}
  MNIST\_FC1 \\
  MNIST\_FC2 \\
  MNIST\_FC3
\end{tabular}&
  \begin{tabular}[c]{@{}c@{}}23329.0 / 94 \\ 107815.86 / 16 \\ 120000 / 0\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}24725.5 / 86\\ \textbf{48650.74} / 61\\ \textbf{100306.86} / \textbf{17}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{7580} / \textbf{99} \\ 80844 / \textbf{83}\\ 118478.55 / 4\end{tabular} 
  &\begin{tabular}[c]{@{}c@{}}29\\26\\1 \end{tabular} \\\hline
15 &
\begin{tabular}{c}
  MNIST\_FC1 \\
  MNIST\_FC2 \\
  MNIST\_FC3
\end{tabular}&
  \begin{tabular}[c]{@{}c@{}}25039.82 / 89 \\ 84655.4 / 32 \\ 120000 / 0\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}8056.5 / 94\\ \textbf{25211.23} / \textbf{79}\\ 120000 / 0 \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{6330} / \textbf{98}\\ 31384.321 / 78 \\ \textbf{118356.89} / \textbf{3}\end{tabular}
  &\begin{tabular}[c]{@{}c@{}}3\\2\\0 \end{tabular} \\\hline
\end{tabular}
}
% \vspace{-5pt}
\end{table}

==> Table_safety-epsilon.tex <==
% \setlength{\textfloatsep}{5pt}
\begin{table}[t]
\centering
\caption{Shows the number of safe and unsafe regions for 10 different networks}
\label{table:safety_regions}
% \begin{minipage}{.3\linewidth}
% \begin{tabular}{|c|c|}
% \hline
% \# of neurons & time(s)\\ \hline
% 1024                    & 3.374           \\ \hline
% 4096                    & 7.2517          \\ \hline
% 20000                   & 7.458           \\ \hline
% 50000                   & 30.189          \\ \hline
% \end{tabular}
% \end{minipage}
% \begin{minipage}{.68\linewidth}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|cccccccccc|}
\hline
Epsilon & \multicolumn{10}{c|}{Number of safe/unsafe regions}         \\ 
        & 1 &2  &3  &4  &5  &6  &7  &8  &9  &10 \\\hline
0.25    &46/52 &33/65 &49/49 &45/53 &46/52 &53/45 &51/47 &63/35 &74/24 &51/47 \\ \hline
0.5     &27/38 &22/43 &30/35 &27/38 &27/38 &29/36 &31/34 &39/26 &49/16 &36/29 \\ \hline
0.75    &20/34  &17/37  &24/30  &21/33  &21/33  &23/31  &26/28  &31/23  &43/11  &32/22 \\ \hline
\end{tabular}}
% \end{minipage}
\end{table} 

%\eps 0.25 [(46, 98), (33, 98), (49, 98), (45, 98), (46, 98), (53, 98), (51, 98), (63, 98), (74, 98), (51, 98), (64, 98), (51, 98)]

%\eps 0.5  [(27, 38), (22, 43), (30, 35), (27, 38), (27, 38), (29, 36), (31, 34), (39, 26), (49, 16), (36, 29), (43, 22), (32, 33)]

%\eps 0.75 [(20, 34), (17, 37), (24, 30), (21, 33), (21, 33), (23, 31), (26, 28), (31, 23), (43, 11), (32, 22), (36, 18), (29, 25)]

==> Table_scalability.tex <==
\begin{table}[t]
% \vspace{-10pt}
% \centering
\caption{\textbf{(Left)}Shows the execution time in seconds for checking the feasibility of transition between a pair of regions in the workspace. We test the scalability of the solver by solving the verification problem for different architectures by varying the number of neurons per layer and the depth of the network. \textbf{(Right)} shows the verification time for single layer networks with different width.}
\label{table:scalability}
\resizebox{.7\textwidth}{!}{%
\begin{tabular}{|c|cccccc|}
\hline
\# of neurons per layer & \multicolumn{6}{c|}{\# of layers}            \\ 
                        & 1       & 2      & 3      & 4      & 5    &6     \\ \hline
20                      & 0.025   & 0.0479 & 0.1184 & 0.4767 & 26.76 &0.257  \\ \hline
128                     &0.267    &1.57        & 243.8 &3394.18         &2740.341 & 1368.55
\\ \hline
256                     & 0.31    & 0.92   &    6956.69    & 136.44 & 4.4352 & 1471.29\\ \hline
512                     & 0.679   & 19.83  & 5.43   &  10058.13     &   9649.55 &35783.58     \\ \hline
\end{tabular}}\qquad
\resizebox{.2\textwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\# of neurons & time(s)\\ \hline
1024                    & 3.374           \\ \hline
4096                    & 7.2517          \\ \hline
20000                   & 7.458           \\ \hline
50000                   & 30.189          \\ \hline
100000                  & 68.8614         \\ \hline

\end{tabular}}
\end{table}




==> Table_singleLayer.tex <==
% \begin{wraptable}{r}{.3\linewidth}
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
\# of neurons & time(s)\\ \hline
1024                    & 3.374           \\ \hline
4096                    & 7.2517          \\ \hline
20000                   & 7.458           \\ \hline
50000                   & 30.189          \\ \hline
\end{tabular}
\end{table}
% \end{wraptable}





==> alg.tex <==
% !TEX root = ../main.tex

\section{Algorithm}
We now describe how our novel search procedure integrates with other techniques 
to form the full PeregriNN algorithm. The state of our algorithm is captured by 
a list of conditioning choices already made. The main loop of the algorithm 
updates this state once per iteration in two sequential stages: a 
\underline{convex query} stage and a \underline{state update} stage. The convex 
query stage entails solving a single convex problem derived from the current 
list of conditioning choices. Based on the result of the convex query, the 
state update stage proceeds in one of two ways: it \underline{conditions} if 
the convex solver returns indeterminate neurons (i.e. descends deeper, adding 
conditionings to the state), or it \underline{backtracks} if the convex solver 
returns infeasible (i.e. ascends shallower, removing conditionings from the 
state). Before executing the convex solver, we also include an 
\underline{inference} step, which further improves efficiency by providing the 
solver additional constraints that are inferred by symbolic interval analysis.

% \g{I think this describes the overall structure of the algorithm. The 
% inter/intra-layer prioritization happens in the conditioning stage -- i.e. 
% which neuron we decide to condition on next. So there we should describe soring 
% the indeterminate neurons by depth, and choose the one with the minimum 
% volume.}

\textbf{Convex Query.} The convex query step takes the current list of 
conditioning choices, and translates them into constraints on the slack 
variables as follows:
\begin{align}
	\text{Neuron } (y_i)_j \text{~ ON: }& \;\;  (y_{i})_j = (W_i y_{i-1} + b_i)_j \wedge (y_{i})_j \geq 0 \label{eq:convex_constraint_1}\\
	\text{Neuron } (y_i)_j \text{ OFF: }& \;\;  (y_{i})_j = 0 \wedge (W_i y_{i-1} + b_i)_j \leq 0.
	 \label{eq:convex_constraint_2}
\end{align}
These constraints are then added of the convex program 
\eqref{eq:peregrinn_convex_program}, and the program is passed to the convex 
solver to solve. The output of the convex solver (for our purposes) is a either 
a list of indeterminate neurons or the conclusion that the program was 
infeasible. Any list of indeterminate neurons returned by the solver does not 
include any of the neurons we have conditioned on already by definition. 
Moreover, any returned indeterminate neurons are at least as deep in the 
network as the last conditioned neuron: this is because of the choice of the 
$q_i$ in \eqref{eq:peregrinn_convex_program} (see 
\cref{sub:intra_layer_prioritization}).

\textbf{State Update.} %
The state update stage proceeds to update the algorithm's state by one of two 
mechanisms, depending on the output of the convex solver.

		\begin{minipage}[t]{\linewidth}
		% begin nowrap
		\parshape 2 10pt \dimexpr\linewidth-10pt 20pt \dimexpr\linewidth-20pt\relax
		% end nowrap
		\textbf{Conditioning.} If the convex solver returns a list of 
		indeterminate neurons, then PeregriNN's unique prioritizations are used 
		to update the state with a new conditioning choice (see 
		\cref{sec:approach}). First, the inter-layer prioritization is applied: 
		the list of indeterminate neurons is sorted by depth, and only those 
		neurons in the layer closest to the input are eligible for 
		conditioning. From these neurons, the next conditioning choice is made 
		using the intra-layer prioritization scheme: the activation region with 
		the smallest volume (that is also compatible with the other 
		conditionings in the layer) is selected, and added to the state. After 
		the state update, a new iteration of the main loop starts.
		\end{minipage}

		\begin{minipage}[t]{\linewidth}
		% begin nowrap
		\parshape 2 10pt \dimexpr\linewidth-10pt 20pt \dimexpr\linewidth-20pt\relax
		% end nowrap
		\textbf{Backtracking.} If the convex solver returns infeasible, then we 
		have explored as far as possible into the network given the current 
		conditioning choices. Thus, the algorithm must backtrack, and undo some 
		of those choices to explore other possible activation combinations. 
		Since each conditioning choice is in direct correspondence with a pair 
		of convex constraints -- i.e. \eqref{eq:convex_constraint_1} and 
		\eqref{eq:convex_constraint_2} -- and the convex solver returned 
		infeasible, we know that these constraints are mutually incompatible. 
		Thus, we can use an Irreducible Inconsistent Subsystem (IIS) of these 
		constraints to find compatible constraints, and roll back some of 
		the conditioning choices in the current state. Moreover, since an IIS 
		is irreducible, 
		% has the property that removing any one constraint 
		% restores feasibility, so we can easily reset the current state to a 
		% feasible set of constraints by this means -- 
		this method often rolls back a considerable number of conditionings at 
		once. After the state update, a new iteration of the main loop starts.
		\end{minipage}

As an additional optimization, we perform an inference step right before 
executing the convex query.

\textbf{Inference.} Given a set of conditioning choices, it is often possible 
to rule out some other neuron activations directly by over-approximation 
methods. Thus, we use Symbolic Interval Analysis\cite{wang2018formal} to find 
other neuron activations that must follow from the current state of 
conditioning choices. These inferred conditioning choices are converted to 
convex constraints as in \eqref{eq:convex_constraint_1} and 
\eqref{eq:convex_constraint_2}, and added to the convex program right before 
the convex query stage is executed.
% This has the effect of improving the quality 
% of the solution returned by the convex solver.

% \vspace{-14pt}
% Proving the assertion in \eqref{Eq:Verification} requires computing the bounds (or the geometric structure in general) of the output $z$ which in turn requires knowing the exact bounds of all the neurons in the network. However, due to the non-linearity, non-convexity of ReLU networks, and the interdependencies between neurons imposed by the structure of the NN, computing such bounds is computationally intractable for modern networks. Specifically, it requires exploring a search space of $2^n$ decisions as will be explained later, but the key challenge is how to explore this search space efficiently.

% % Davis–Putnam–Logemann–Loveland (DPLL) algorithm is an efficient and complete backtracking-based search algorithm that checks the satisfiability of  propositional logic formulae which is an NP-complete problem. It is known\cite{Relu} that the NN verification problem can be easily reduced to the SAT problem and hence it is an NP-complete problem too. In the footsteps of DPLL, we propose a principled NN model checker based on three main steps which are \textit{conditioning, inference,} and \textit{backtracking}. To explain each of these steps, we first define the phase of a ReLU as the region in which the ReLU is operating. More precisely, we say that neuron $(i,j)$ is \textbf{active} if $\hat{y}_{ij} \geq 0$, and we say it's \textbf{inactive} if $\hat{y}_{ij} \leq 0, \,\forall \hat{y}_{ij}$ satisfying \eqref{Eq:network}.

% We use Symbolic Interval Analysis\cite{wang2018formal} for estimating over approximated bounds on the output of each neuron. These bounds are function of the network input $x$. We denote the bound equations of $\hat{y}_{ij}$ and $y_{ij}$ by $\hat{Eq}_{ij}(x)$ and ${Eq}_{ij}(x)$ respectively for neuron $n_{ij}$ and hence we can compute the approximate lower and upper bounds of  $\hat{y}_{ij}$ denoted by  $\hat{l}_{ij} = \min_{x} \hat{Eq}_{ij}(x)$ and  $\hat{u}_{ij}=\max_{x} \hat{Eq}_{ij}(x)$
% % \begin{equation}
% %     \begin{aligned}
% %     \hat{l}_{ij} &= \min_{x} \hat{Eq}_{ij}(x) \,\leq \min_{x} \hat{y}_{ij}\\
% %     \hat{u}_{ij} &= \max_{x} \hat{Eq}_{ij}(x) \geq \max_{x} \hat{y}_{ij} 
% %     \end{aligned}
% % \end{equation}
% % approximate bounds on $y_{ij}$ can be computed similarly. 
% \paragraph{Conditioning.}
% Since the ReLU function is piece-wise linear, we define the phase of the neuron as the region in which the ReLU is operating. More precisely, we say that neuron $n_{ij}$ is \textbf{active} if $\hat{y}_{ij} \geq 0, \,\forall \hat{y}_{ij}$ satisfying \eqref{Eq:network}, and we say it's \textbf{inactive} if $\hat{y}_{ij} \leq 0, \,\forall \hat{y}_{ij}$ satisfying \eqref{Eq:network}. Using these bounds we define the sets $\Gamma_{i}^{+} = \{j \mid \hat{l}_{ij} \geq 0\}$, $\Gamma_{i}^{-} = \{j \mid \hat{u}_{ij} \leq 0\}$, and $\Gamma_{i} = \{j \mid \hat{l}_{ij} \leq 0 \leq \hat{u}_{ij}\}$
% where $\Gamma_{i}^{+}$ and $\Gamma_{i}^{-}$ are the sets of active and inactive nodes respectively, and $\Gamma_{i}$ is the set of \textbf{undecided} neurons which are neither active or inactive.
% At each iteration of the algorithm we solve a relaxed convex program\eqref{eq:simple_relaxed_convex} with slacked objective, and get an approximate solution. This is the Inter layer prioritization step. To further refine this solution, we fix the phase of one of the neurons which minimizes the volume of the input space as part of the intra layer prioritization step. We do this iteratively to tighten the convex program and resolve it until we get an exact solution. 
% % Just like the SAT problem and the DPLL algorithm, the choice and ordering of these decisions highly affect the exploration of the search space and hence the performance. The key challenge is to find the smallest sequence of decisions(neurons to fix) that leads us to the solution or to conclude infeasibility.
 
% % Since conditioning on any of the neurons partitions the input space with a hyperplane, we choose to condition on the neuron which minimizes the volume of the input space. Moreover, conditioning on a neuron in earlier layers strongly affects the bounds of the network and the output and leads to a much tighter problem. Therefore, we encourage the solver to condition on a neuron in the earlier layers of the network that minimizes the volume of the input space.
% \vspace{-5pt}
% \paragraph{Inference.}
% Fixing the phase of one of the neurons in layer $i$ affects the approximate bounds of all subsequent neurons in layer $k, \;i< k\leq n$. For example, forcing a certain neuron to be inactive by conditioning on it, may force another neuron to also be inactive. In the inference step, we recompute the bounds equations $\hat{Eq}_{kj}(x),Eq_{kj}(x)$ and using the updated bounds we infer whether any of the nodes must be active or inactive. Inferring those decisions in turn tightens the bounds of the outputs and constrain the convex problem, making it easier to find a solution or conclude infeasibility.
% % This step is analogous to the unit resolution step(setting the free literal to true) in DPLL, in the sense that whenever we fix a neuron we are enforcing constraints on other neurons by updating their bounds.
% \vspace{-5pt}
% \paragraph{Backtracking.}
% After conditioning on a set of neurons, the relaxed convex problem may be infeasible. This infeasibility might be because the property we are verifying holds and there doesn't exist a solution to violate the property, or because we have made a wrong decision when conditioning on one of the neurons. For the latter case we need to backtrack and change one of the decision we made to continue exploring the search space. Using vanilla Depth First Search (DFS) is not very efficient as it doesn't have any mechanism of determining the actual reason of infeasibility. Since we add a hyperplane constraint whenever we condition on a neuron, we rely on the convex solver to compute the Irreducible Inconsistent Subsystem (IIS) on these hyperplane constraints and then backtrack to the neuron in the IIS that we last conditioned on. The IIS is the set of constraint such that if any of those constraints is removed from the problem it becomes feasible again. This allows us to backtrack several steps during the search and hence avoid unneeded exploration.

 


% We approach this by trying to falsify assertion \eqref{Eq:Verification} by solving a relaxed convex program in \eqref{Pb:Relaxed} using approximate bounds. The solution to the convex program might not be exact due to the relaxation and it might not satisfy the NN constraints in \eqref{Eq:network}, so whenever we get a solution for the convex program we check if it satisfies \eqref{Eq:network}, if not, then we tighten the approximate bounds by fixing the phase of one of the neurons and updating the bounds of all other neurons. We then repeat this process iteratively by solving a tighter convex program using the updated bounds then tighten these bounds until we get a solution that satisfies \eqref{Eq:network} or conclude that the property actually holds if we can't find a solution that violates the property.

% To construct the convex program, we use ReLU convex relaxation proposed by Ehler et al.\cite{Planet} as shown in figure \ref{Fig:ReluRelaxed}. Consider a single ReLU with input lower and upper bounds $\hat{l}$ and $\hat{u}$ respectively, using this relaxation $y = ReLU(\hat{y}) = max(0,\hat{y})$ can be relaxed to the set of linear constraints 
% \begin{equation}
%     % \begin{aligned}
%         y \geq 0,\;
%         y \geq \hat{y},\;
%         y \leq \frac{\hat{u}}{\hat{u} - \hat{l}}(\hat{y} -\hat{l})
%     % \end{aligned}
% \end{equation}
% We estimate the lower and upper bounds using Symbolic Interval Analysis\cite{ReluVal} which gives tight bounds in a computationally efficient way.

% Using this relaxation we attempt to falsify the property of interest by solving the relaxed convex program
% \begin{equation}
%     \begin{aligned}
%     \min_{x,\hat{y}_1,..,\hat{y}_n,y_1,..,y_n}&\quad  \sum_{i=1}^n\sum_{j\in\Gamma_{i}} q_i y_{ij}\\
%     \textrm{s.t.}\quad& y_{ij} = 0, \; \forall j \in \Gamma_{i}^{-} \\
%     \quad& y_{ij} = \hat{y}_{ij}, \; \forall  j \in \Gamma_{i}^{+} \\
%     y_{ij}\geq 0,\;&y_{ij}\geq \hat{y}_{ij}, \;y_{ij} \leq \frac{\hat{u}_{ij}}{\hat{u}_{ij} - \hat{l}_{ij}}(\hat{y}_{ij} -\hat{l}_{ij}),\; \forall j \in \Gamma_{i}\\
%     \quad& \hat{y}_i = W_i y_{i-1} + b_i\\
%     \quad& x\in R_x,\; z\in R_z^\mathsf{c}
%     \end{aligned}
%     \label{Pb:Relaxed}
% \end{equation}
% where $R_z^\mathsf{c}$ is the complement of $R_z$ and $q_i$ is an optimization weight which is used to penalize non-zero ReLUs in some layers more than others. The usage of $q_i$ is described later in the algorithm section.

% If there is no solution to \eqref{Pb:Relaxed} then the property holds, if there is a solution that satisfies \eqref{Eq:network} then the property is violated and a counterexample is found. However, if there exists a solution that doesn't satisfy \eqref{Eq:network} then we fix the phase of one of the neurons and update the network bounds. Fixing the phase of a neuron is equivalent to adding one of the following constraints to \eqref{Pb:Relaxed}
% \begin{equation}
%     c_{ij}=\begin{cases}
%             \begin{aligned}
%               \hat{Eq}(x) \leq 0 \; \land \; y_{ij} = 0 \qquad\quad\Gamma_{ij} =\text{inactive}\\
%               Eq(x) = \hat{Eq}(x)\; \land \; y_{ij} = \hat{y}_{ij} \quad \Gamma_{ij} = \text{active}
%             \end{aligned}
%           \end{cases}
%     \label{Eq:BoundsCnstrnts}
% \end{equation}
% \text{where} $\Gamma_{ij}$ \text{ is the decided phase for neuron}$n_{ij}$

% In the worst case, to find a solution that satisfies \eqref{Eq:network} or conclude that the property holds we'll need to search over all possible $2^n$ enumerations of phases of the neurons which is impractical for modern networks. Our approach uses the solution of the convex optimizer and a set of heuristics to guide our search and prune the search the space as early as possible.

% \subsection{Conditioning}
% We use the solution to the relaxed convex optimization problem as a guide for conditioning. More specifically, we define a candidate set $C = \{(i,j) \mid y_{ij} > max(0,\hat{y}_{ij})\}$ which is the set of neurons with solutions (from solving the relaxed problem) not lying on the ReLU function. We then condition on one of those neurons $(i,j)\in C$. We encourage the solver to find a candidate set $C$ of neurons in the earlier layers by choosing $q_i$ in \eqref{Pb:Relaxed} to be increasing with $i$ to penalize infeasibility of neurons in later layers

% \subsection{Inference}
% In the inference step, we recompute the bound equations $\hat{Eq}_{kj}$ and we add $j$ to $\Gamma_k^+$ if $\hat{l}_{kj} \geq 0$ or to $\Gamma_k^-$ if $\hat{u}_{kj} \leq 0$.
% \subsection{Backtracking}
% \begin{wrapfigure}{R}{0.7\textwidth}
% \begin{minipage}{0.7\textwidth}
\setlength{\textfloatsep}{5pt}
\begin{algorithm}[t]
\small
    \begin{algorithmic}[1]
    \Procedure{NN\_verify}{nn, problem}
    \State inferred = $\phi$; decided = $\phi$
    \While{True}
    \State inferred, undecided $\gets$ \Call{SymIntervalAnalysis}{nn, problem.input\_bounds}
    \State sol, realxed\_neurons$\gets$\Call{CheckFeas}{nn, problem, undecided} \Comment{Inter layer prioritization}
        \If{sol.status == INFEASIBLE} 
           
           \If{decided == $\phi$} \Return SAFE
           \Else
            \State decided $\gets$ \Call{backtrack}{decided, problem}
           \EndIf
        \ElsIf{$|$relaxed\_neurons$|$ == 0}
            \Return UNSAFE, sol
        \Else
        % \State sol$\gets$\Call{dfs}{nn, problem, realxed\_neurons}
         \State neuron $\gets$\Call{pick\_one}{relaxed\_neurons} \Comment{Intra layer prioritization}
         \State decided $\gets$ decided $\bigcup$ neuron
         
        %  \State \textbf{return} sol.status, sol 
        % \Comment{INFEASIBLE$\iff$SAFE}
        \EndIf
    \EndWhile

    % \EndProcedure
    % \Statex
    % \Procedure{DFS}{nn, problem, realxed\_neurons}
    % \State neuron $\gets$\Call{pick\_one}{realxed\_neurons}
    
    % % \Comment{that minimizes the volume of input space}
    
    % \State \Call{fix\_phase}{nn, neuron, phase, problem}
    % \State sol, realxed\_neurons$\gets$\Call{CheckFeas}{nn,problem}
    % \If{sol.status == FEASIBLE}
    
    %     \If{$|$realxed\_neurons$|$ == 0}
        
       
    %         \State\Return sol
    %         % \Comment{neurons lie on ReLU}
    
    
    %     \Else
    %         \State sol$\gets$\Call{dfs}{nn,problem,realxed\_neurons}
    %     \EndIf
    % \EndIf
    
    % \If{sol.status == INFEASIBLE}
    
    % \State\Call{fix\_phase}{nn, neuron, $\neg$phase, problem}
    
    % \State sol$\gets$\Call{dfs}{nn,problem,realxed\_neurons}
    % \EndIf
    % \State \textbf{return} sol
    
    \EndProcedure
\end{algorithmic}
 \caption{Verification of ReLU networks}
 \label{Alg:NN_verify}
\end{algorithm}
% \end{minipage}
% \end{wrapfigure}




==> approach.tex <==
% !TEX root = ./main.tex

\section{Approach} % (fold)
\label{sec:approach}

% Text from old abstract -- suitable for introduction
%
% However, we introduce a novel approach to resolve indeterminate neuron 
% activations that confers a number of unique advantages. In particular, we 
% condition on these neurons in order of depth from input layer to output layer, 
% so that each such neuron may be regarded as an input neuron in its own right, 
% whose input comes from a network operating in a linear region. This is an 
% advantageous paradigm for two reasons: one, input neurons have activation 
% regions with a much simpler geometry (indeed, they are half-spaces); and two, 
% the layers containing indeterminate neurons always receive inputs for which 
% exact bounds are available. 
\begin{wrapfigure}[11]{r}{0.31\textwidth} %[H] %
    %\vspace{-19mm}
	\centering 
	\includegraphics[width=0.31\textwidth]{neuron_response_slack.pdf} 
	\caption{Neuron activation by minimizing a slack variable, $y_i$.}
	\label{fig:valid_activation}
\end{wrapfigure}
As in some other algorithms, we convert the verification problem 
(\cref{sec:problem_formulation}) into a relaxed convex program (e.g. 
% begin nowrap
\cite{wang2018efficient,wang2018formal,bunel2020branch}). 
% end nowrap
Convex programs of this type assign a slack variable to the output of each 
neuron that is purposely allowed to differ from the actual output of the neuron 
(as calculated from its inputs). Each slack variable is then constrained to lie 
above the response of its associated neuron, and the input and output sets from 
the verification problem are incorporated as further constraints on the 
relevant slack variables. The objective, then, is to minimize the sum of total 
slacks in the hope that each slack variable will be driven to lie 
\emph{exactly} on the response of its respective neuron. In such a case, the 
solver will have found a solution that corresponds to an actual input/output 
pair for the network, and thus decide the verification problem. Mathematically, 
relaxed convex programs of this type can be written as:
%have the following general form:
\begin{equation}
	\min_{y_0,..,y_n}  \sum_{i=0}^n\sum_{j=1}^{k_i} y_{ij}
	\quad \text{s.t.} \quad
	\begin{cases}
		y_{i}\geq 0, \;
		y_i \geq W_i y_{i-1} + b_i &\forall i = 1, \dots, n \\
		y_0 \negthinspace \in \negthinspace P_{y_0},\;
		y_n \negthinspace \in \negthinspace P_{y_n}, \;
		\underset{\ell=1}{\overset{m}{\wedge}} h_\ell(y_0,y_n) \leq 0 & ~
	\end{cases}
	\label{eq:simple_relaxed_convex}
\end{equation}
A valid input/output pair for the network is obtained when either $y_i=0$ or 
$y_i=W_i y_{i-1} + b_i$ for all $i = 1, \dots, n$. An example of this situation 
is depicted in \cref{fig:valid_activation}, where the black dot illustrates a 
choice of the slack variable $y_i$ that corresponds to a valid input/output 
pair for the illustrated neuron.

Given the efficiency of modern convex solvers, this is an extremely attractive 
approach when it is successful. However, all formulations of this type suffer 
from the same drawback: the solver may return a solution in which some of the 
slack variables are \emph{indeterminate} -- i.e. they do not lie on the 
response of their respective neurons. In a case like this, the solution doesn't 
correspond to an actual evaluation of the network, and more work is needed to 
decide the verification problem. In particular, the indeterminate neurons must 
be \emph{conditioned} -- i.e. constrained to be either active or inactive -- 
and then the convex program re-solved with these new constraints. This process 
is repeated as a search over all combinations of different conditionings until 
either a valid solution is found or the problem is shown to be infeasible.

The primary novelty in our approach is thus the way in which we search over the 
different possible conditionings of indeterminate neurons. Most approaches 
treat all indeterminate neurons as roughly equivalent for the purpose of 
search, and use ReLU over-approximation methods to guide which neuron to 
consider next (and to exclude combinations when possible). Instead, we propose 
a new, more efficient heuristic that prioritizes neurons in a way that 
emphasizes the \emph{geometry of their activation regions}: our approach uses 
this information to more effectively exclude combinations of conditionings from 
the search space. Our approach has two specific levels of prioritization that 
we described subsequently.

		% \begin{minipage}[t]{\linewidth}
		% % begin nowrap
		% \parshape 2 10pt \dimexpr\linewidth-10pt 20pt \dimexpr\linewidth-20pt\relax
		% % end nowrap
		% \textbf{(1) Inter-layer Prioritization.} We always prioritize 
		% conditioning neurons from layers that are closest to the input layer. 
		% In some cases, this simple rule automatically excludes all but a 
		% \emph{sub-exponential} number of combinations of neurons in each layer, 
		% based purely on the geometry of the neurons' activation regions. Even 
		% in general cases, though, this prioritization method achieves 
		% significant savings for similar geometric reasons.
		% \end{minipage}\\[5pt]
		% \begin{minipage}[t]{\linewidth}
		% % begin nowrap
		% \parshape 2 10pt \dimexpr\linewidth-10pt 20pt \dimexpr\linewidth-20pt\relax
		% % end nowrap
		% \textbf{(2) Intra-layer Prioritization.} We can also exploit the 
		% geometric properties of neurons' activation regions to prioritize 
		% conditionings within a layer. We prioritize neurons based on the volume 
		% of their activation regions: this heuristic balances the accuracy of 
		% ReLU over-approximation methods with their ability to exclude 
		% combinations of conditionings in order to exclude yet more combinations 
		% of conditionings.
		% \end{minipage}

\begin{wrapfigure}[34]{r}{0.35\textwidth}
	%\vspace{-12mm}
	\centering
	\begin{tabular}{ c }
		\includegraphics[width=0.30\textwidth]{hidden_neuron_activation.pdf} 
		\\[2pt]
		\includegraphics[width=0.34\textwidth]{neuron_selection_order.pdf}
	\end{tabular} %\vspace{-4mm}
	\caption{ %
	\textbf{(Top)} Activation regions for a three-neuron NN with a 2-d 
	\emph{input-feature space}. The NN has two input neurons and one output 
	neuron: black and red lines show activation boundaries for input neurons; 
	the blue line shows the activation region for the output neuron. %
	\textbf{(Bottom)} Illustration of the conditioning order. Indeterminate 
	neurons are shown in blue, with those already conditioned also filled-in; 
	all other neurons are active or inactive as specified by the convex solver. 
	The next neuron is selected from the red rectangle. %
	}
	\label{fig:inter-layer_illustration}
\end{wrapfigure}

\subsection{Inter-Layer Prioritization} % (fold)
\label{sub:inter-layer_prioritization}

% The benefit of always conditioning on a neuron in the input layer (of some 
% un-conditioned network as shown in \cref{fig:inter-layer_illustration}) has to 
% do with the geometry of their activation regions.

Consider neurons' activation regions as expressed in the input-feature space of 
a network: the activation regions of input-layer neurons are always 
hyperplanes, whereas the activation regions for deeper neurons are more 
complicated regions -- see the top pane of \cref{fig:inter-layer_illustration} 
for an example. Thus, input-neuron activation regions are specifically subject 
to all of the geometric properties of \emph{hyperplane arrangements} 
\cite{StanleyIntroductionHyperplaneArrangements}. In particular, the geometric 
properties of hyperplane arrangements govern which input-layer-neuron 
activation regions have non-empty intersections, and hence which combinations 
of activations are simultaneously possible. In the extreme case when there are 
more neurons in an input layer than there are inputs, the reduction in possible 
activation combinations can be considerable. It is known that in such cases, 
the number of non-empty regions formed by an arrangement of hyperplanes scales 
\emph{sub-exponentially} in the number of hyperplanes -- i.e. the number of 
input-layer neurons. In particular, the number of regions formed by $N$ such 
hyperplanes each of dimension $n$ is at most $\sum_{i = 0}^{n} 
{\genfrac{(}{)}{0pt}{}{N}{i}}$.

Thus, we propose to always condition on those indeterminate neurons closest to 
the input layer, since this will recreate these geometric properties for all 
indeterminate neurons within the same layer -- even if that layer is deeper in 
the network. Spurious conditionings can thus be eliminated by evaluating the 
compatibility of these indeterminate neurons according to their 
activation-region hyperplanes \emph{before} conditioning them. This amounts to 
a direct pruning of conditionings from the search space. Note that the 
sub-exponential savings is particularly salient in shallow networks where the 
number of neurons typically exceeds the number of inputs by a significant 
factor.

This prioritization works because it effectively partitions the network along a 
layer boundary into two sub-networks: see the bottom pane of 
\cref{fig:inter-layer_illustration}. The suggestively named fixed-phase 
sub-network necessarily operates in a (known) linear region because the phases 
of all of its neurons are fixed (either by the convex solver or already taken 
conditioning decisions). Consequently, the relevant portion of the input 
constraint set can be propagated through this fixed-phase sub-network to obtain 
an exact polytope representation of its outputs. But the next indeterminate 
neuron to be conditioned can be regarded as belonging to the input layer of the 
un-conditioned sub-network, whose input is of course supplied by the output  of 
the fixed-phase sub-network. Thus, we can effectively reconsider the original 
verification problem in terms of a new verification problem on the 
un-conditioned sub-network, and one where next indeterminate neuron to be 
conditioned is in the input layer.

There is one important implementation detail that is necessary to actually 
implement this layer-wise prioritization, but which we have not yet mentioned. 
Notably, the search procedure involves re-solving the convex program with 
neuron conditionings as we decide them, and in general, this may result in new 
indeterminate neurons in layers closer to the input layer than the last neuron 
we conditioned. In order to prevent this, and thus ensure that re-solving the 
convex program forces new indeterminate neurons to appear deeper in the 
network, we modify the objective function in \eqref{eq:simple_relaxed_convex} 
with layer-wise weights that strongly penalize slacks in earlier layers. That 
is we use an objective function like:
\begin{equation}\label{eq:peregrinn_convex_program}
	\min_{y_0,..,y_n}  \sum_{i=0}^n\sum_{j=1}^{k_i}  q_i y_{ij}
	\quad \text{s.t.} \quad
	\begin{cases}
		y_{i}\geq 0, \;
		y_i \geq W_i y_{i-1} + b_i &\forall i = 1, \dots, n \\
		y_0\in P_{y_0},\;
		y_n\in P_{y_n}^\mathsf{c}, \;
		\underset{\ell=1}{\overset{m}{\wedge}} h_\ell(y_0,y_n) \leq 0 & ~
	\end{cases}
\end{equation}
where the coefficients $q_1 \ll q_2 \ll \dots \ll q_n$ are chosen so that 
non-zero slack variables are guaranteed to be driven as close to the input 
layer as possible using the notion of prefix-ordered monotone formulas shown in \cite{ShoukrySMCSatisfiabilityModulo2018}.


% The most crucial point of distinction is that we take an \emph{input-space} 
% point of view to conditioning indeterminate neurons (as opposed to conditioning 
% based on the influence of a neuron on the output). In particular, we know that 
% because the number of hyperplanes in an arrangement scales sub-exponentially, 
% we don't have to consider all permutations of conditionings in general. 
% Moreover, incompatible conditionings can generally be found easily by means of 
% a convex solver that returns IISs.



% subsection inter_layer_prioritization (end)

\subsection{Intra-Layer Prioritization} % (fold)
\label{sub:intra_layer_prioritization}

One important technique to improve the conditioning search is to use ReLU 
over-approximations (e.g. symbolic interval 
% begin nowrap
analysis~\cite{zhang2018efficient,wang2018formal}) 
% end nowrap
to show that a particular conditioning cannot possibly satisfy 
the constraints of the verification problem. That is if the over-approximation 
can't satisfy the output constraints, then the particular choice of 
conditioning can't either. Over-approximations of this type are best be 
employed when not all of the neurons have yet been conditioned: if a particular 
neuron conditioning is impossible, then there is no need to check the 
activation combinations of the \emph{remaining} indeterminate neurons. The 
opposite conditioning can thus be incorporated into the convex program as a 
constraint to aid the convex solver the next time it is run. In particular, 
when a specific indeterminate neuron can be shown to necessarily be on or off, 
the inequality constraints for that neuron in \eqref{eq:simple_relaxed_convex} 
can be replaced by the combined constraints $(y_{i})_j = (W_i y_{i-1} + b_i)_j 
\wedge (y_{i})_j \geq 0$ or $(y_{i})_j = 0 \wedge (W_i y_{i-1} + b_i)_j \leq 
0$, respectively.

However, over-approximations like this come with a drawback: the more neurons 
that can be both active and inactive in a region, the worse the approximation 
error is -- and hence the less likely that that particular combination is 
invalidated by the over-approximation. On the other hand, the more neurons that 
have both phases active in a region, the more possible combinations that are 
eliminated if the activation region \emph{is} infeasible. Thus, there would seem to be an 
intuitive trade-off between the number of further conditionings that are 
possible within an activation region, and the likelihood that those 
combinations can be excluded by over-approximating the network.

Given the need to use over-parameterized deep networks for effective training, 
it is plausible to suppose that activation regions are roughly uniformly 
distributed within any un-conditioned network (as defined in 
\cref{fig:inter-layer_illustration}). According to this heuristic, then, the 
\emph{volume} of an activation region is a useful proxy for the number of 
indeterminate neurons that can be excluded by over-approximating the network on 
that region. This volume heuristic is an especially convenient one given the 
discussion above: after all, it is considerably easier to compute the volume of 
activation regions when those activation regions are defined by hyperplanes, as 
they are for neurons in the input layer; again, refer the top pane of 
\cref{fig:inter-layer_illustration}.

% The geometric arguments 
% above to suggest a useful, efficient heuristic that trades off between these 
% competing factors. 

Thus, we start from the observations in \cref{sub:inter-layer_prioritization} 
to propose the following intra-layer conditioning priority: we condition the 
next indeterminate neuron (within a layer) according to the (valid) activation 
region that has the \emph{smallest volume}. We reiterate that this heuristic is 
only reasonable to implement because of the geometric basis we established 
above. Moreover, we have found that minimum-volume priority is an effective 
heuristic across all of our experiments, which suggests that the aforementioned 
trade-off skews heavily toward the accuracy of the over-approximation, not the 
number of neurons that can be excluded. Nevertheless, this analysis suggests 
that there is a rich opportunity for future work here. In particular, it is 
natural to consider the possibility of a volume-based prioritization that is 
adaptive according to the properties of the individual neuron under 
consideration.

% his heuristic works so well suggests 
% that at least for many common networks, it is much more important to get 
% accurate over-approximations than it is to try loose over-approximations that


% This heuristic is first and foremost only possible because of the geometric 
% arguments outlined in \cref{sub:inter-layer_prioritization}: indeed as 
% \cref{fig:inter-layer_illustration} shows, it is difficult to obtain the volume 
% of activation regions when those neurons are not in the input layer. 
% Conversely, it is relatively easy to compute the volume of input-layer 
% activation regions which split the input polytope constraint along two 
% half-spaces. Moreover, the fact that 

% 	\begin{enumerate}
% 		\item The number of potential combinations that are invalidated 
% 			by means of over-approximating the output of the network based 
% 			on a particular conditioning as it implies a constraint on the 
% 			input space; and

% 		\item the likelihood of obtaining an invalidation on such a 
% 			region by means of the symbolic arithmetic over-approximation.
% 	\end{enumerate}
% Thus, we propose a ``minimal-volume conditioning'' heuristic as a way of 
% prioritizing input regions created by conditionings of indeterminate neurons.

% subsection intra_layer_prioritization (end)


% section approach (end)






























==> broader_impact.tex <==
% !TEX root = ../main.tex

\section*{Broader Impact} % (fold)
\label{sec:broader_impact}
New advances in AI systems have created an urgency to study safety, reliability, and potential problems that can rise and impact the society by the deployment of AI-enabled systems in the real world. Mathematically based techniques for the specification, development, and verification of complex systems, also known as formal methods, hold the promise to provide appropriate rigorous analysis of the reliability and safety of such AI-enabled systems.

This work provides a new solver to formally verify whether a NN satisfies specified formal properties in a bounded model checking scheme. The basic idea of bounded model checking is to search for a counterexample that violate the formal property. Such counterexamples can be then used by NN  developers to better understand the limitations of the trained NN in terms of safety, robustness, and hopefully bias. This in turn can enable the use of AI in safety critical cyber-physical applications that are generally regarded to have positive societal influences: autonomous cars and aircraft collision avoidance systems, for example.
% increase safety -- both 
% inherently and with respect to malicious attacks -- of a number of technologies 
% that are generally regarded to have positive societal influences: autonomous cars and aircraft collision avoidance systems, for example.
This work can also be used to identify performance and robustness problems in NNs that are used in non-cyber-physical applications: for example, NNs that are used in criminal justice contexts or to decide creditworthiness.
%
On the negative side, formally verified AI systems may result into a false sense of safety since such technologies do not reason about un-modeled behaviors and side-effects. Another negative effect stems from the proliferation of the technologies that it enables: for example, increased deployment of autonomous vehicles has the potential to cause job loss.

% result into larger adaptations of AI technologies that may have negative societal side-effects

% We expect our algorithm to be used mostly to 
% verify properties that reflect the safety of the NN, especially in the context 
% of cyber-physical systems. However, this work also finds application in 
% verifying the robustness of NNs to corrupted or biased training data, 
% adversarial inputs or both.

% The broader societal impacts of this work are potentially both positive and 
% negative. On the positive side, this work promises to increase safety -- both 
% inherently and with respect to malicious attacks -- of a number of technologies 
% that are generally regarded to have positive societal influences: autonomous 
% cars and aircraft collision avoidance systems, for example. This work can also 
% be used to identify performance and robustness problems in NNs that are used in 
% non-cyber-physical applications: for example, NNs that are used in criminal 
% justice contexts or to decide creditworthiness. The negative externalities of 
% this work stem mostly from the proliferation of the technologies that it 
% enables: for example, increased deployment of autonomous vehicles has the 
% potential to cause job loss.


% Authors are required to include a statement of the 
% broader impact of their work, including its ethical aspects and future societal 
% consequences. Authors should discuss both positive and negative outcomes, if 
% any. For instance, authors should discuss a) who may benefit from this 
% research, b) who may be put at disadvantage from this research, c) what are the 
% consequences of failure of the system, and d) whether the task/method leverages 
% biases in the data. If authors believe this is not applicable to them, authors 
% can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

% section broader_impact (end)
